Calibration of the NEXT-White detector using $^{83m}\mathrm{Kr}$ decays

The NEXT-White (NEW) detector is currently the largest radio-pure high-pressure xenon gas time projection chamber with electroluminescent readout in the world. NEXT-White has been operating at Laboratorio Subterr\'aneo de Canfranc (LSC) since October 2016. This paper describes the calibrations performed with $^{83m}\mathrm{Kr}$ decays during a long run taken from March to November 2017 (Run II). Krypton calibrations are used to correct for the finite drift-electron lifetime as well as for the dependence of the measured energy on the event position which is mainly caused by variations in solid angle coverage. After producing calibration maps to correct for both effects we measure an excellent energy resolution for 41.5 keV point-like deposits of (4.553 $\pm$ 0.010 (stat.) $\pm$ 0.324 (sys.)) % FWHM in the full chamber and (3.804 $\pm$ 0.013 (stat.) $\pm$ 0.112 (sys.)) % FWHM in a restricted fiducial volume. Using naive 1/$\sqrt{E}$ scaling, these values translate into resolutions of (0.516 $\pm$ 0.0014 (stat.) $\pm$ 0.0421 (sys.)) % FWHM and (0.4943 $\pm$ 0.0017 (stat.) $\pm$ 0.0146 (sys.)) % FWHM at the $Q_{\beta\beta}$ energy of xenon double beta decay (2458 keV), well within range of our target value of 1%.

==> pool/NextAuthorList/NextAuthorListMarch_2018.tex <==
\collaboration{The NEXT Collaboration}

\author[a]{C.~Adams,}
%
\author[b]{V.~\'Alvarez,}
%
\author[c]{L.~Arazi,}
%
\author[d]{C.D.R.~Azevedo,}
%
\author[n]{K. Bailey,}

\author[b]{J.M.~Benlloch-Rodr\'{i}guez,}
%
\author[e]{F.I.G.M.~Borges,}
%
\author[b]{A.~Botas,}
%
\author[b]{S.~C\'arcel,}
%
\author[b]{J.V.~Carri\'on,}
%
\author[f]{S.~Cebri\'an,}
%
\author[e]{C.A.N.~Conde,}
%
\author[b]{J.~D\'iaz,}
%
\author[g]{M.~Diesburg,}
%
\author[e]{J.~Escada,}
%
\author[h]{R.~Esteve,}
%
\author[b]{R.~Felkai,}
%
\author[i]{L.M.P.~Fernandes,}
%
\author[j, t, b]{P.~Ferrario,}
%
\author[d]{A.L.~Ferreira,}
%
\author[i]{E.D.C.~Freitas,}
%
\author[j]{J.~Generowicz,}

\author[k]{A.~Goldschmidt,}
%
\author[j, t, b,1]{J.J.~G\'omez-Cadenas,\note{\label{note1}NEXT Co-spokesperson.}}
%
\author[l]{D.~Gonz\'alez-D\'iaz,}
%
\author[a]{R.~Guenette,}
%
\author[m]{R.M.~Guti\'errez,}
%
\author[n]{K.~Hafidi,}
%
\author[o]{J.~Hauptman,}
%
\author[i]{C.A.O.~Henriques,}
%
\author[m]{A.I.~Hernandez,}
%
\author[l]{J.A.~Hernando~Morata,}
%
\author[h]{V.~Herrero,}
%
\author[n]{S.~Johnston,}
%
\author[p]{B.J.P.~Jones,}
%
%
\author[b]{M.Kekic,}
%
\author[q]{L.~Labarga,}
%
\author[b]{A.~Laing,}
%
\author[g]{P.~Lebrun,}
%
%\author[b]{I.~Liubarsky,}
%
\author[b]{N.~L\'opez-March,}
%
\author[m]{M.~Losada,}
%
\author[a]{J.~Mart\'in-Albo,}
%
\author[l]{G.~Mart\'inez-Lema,}
%
\author[b]{A.~Mart\'inez,}
%
\author[p]{A.D.~McDonald,}
%
\author[p, j]{F.~Monrabal,}
%
\author[i]{C.M.B.~Monteiro,}
%
\author[h]{F.J.~Mora,}
%
%\author[d]{L.M.~Moutinho,}
%
\author[b]{J.~Mu\~noz Vidal,}
%
\author[b]{M.~Musti,}
%
\author[b]{M.~Nebot-Guinot,}
%
\author[b]{P.~Novella,}
%
\author[p,1]{D.R.~Nygren, }
%
\author[b]{B.~Palmeiro,}
%
\author[g]{A.~Para,}
%
\author[b]{J.~P\'{e}rez,}
%
\author[b]{M.~Querol,}
%
\author[b]{J.~Renner,}
%
\author[n]{J.~Repond,}
%
\author[n]{S.~Riordan,}
%
\author[r]{L.~Ripoll,}
%
\author[b]{J.~Rodr\'iguez,}
%
\author[p]{L.~Rogers,}
%

\author[b]{C.~Romo,}

\author[e]{F.P.~Santos,}
%
\author[i]{J.M.F.~dos~Santos,}
%
\author[b, c]{A.~Sim\'on,}
%
\author[s,2]{C.~Sofka,}
%
\author[b]{M.~Sorel,}
%
\author[s]{T.~Stiegler,}
%
\author[h]{J.F.~Toledo,}
%
\author[b]{J.~Torrent,}
%
%\author[t]{Z.~Tsamalaidze,}
%
\author[d]{J.F.C.A.~Veloso,}
%
\author[s]{R.~Webb,}
%
\author[s,2]{J.T.~White,\note{Deceased.}}
%
\author[b]{N.~Yahlali}
%

\note{NEXT Co-spokesperson.}
\note{Deceased.}

\emailAdd{next-src@pegaso.ific.uv.es}


%
\affiliation[a]{
  Department of Physics, Harvard University\\
  Cambridge, MA 02138, USA}
%
\affiliation[b]{
Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia\\
Calle Catedr\'atico Jos\'e Beltr\'an, 2, 46980 Paterna, Valencia, Spain}
%
\affiliation[c]{
  Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev\\
P.O.B. 653 Beer-Sheva 8410501, Israel}
%
\affiliation[d]{
Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro\\
Campus de Santiago, 3810-193 Aveiro, Portugal}
%
\affiliation[e]{
LIP, Department of Physics, University of Coimbra\\
P-3004 516 Coimbra, Portugal}
%
\affiliation[f]{
Laboratorio de F\'isica Nuclear y Astropart\'iculas, Universidad de Zaragoza\\ 
Calle Pedro Cerbuna, 12, 50009 Zaragoza, Spain}
%
\affiliation[g]{
Fermi National Accelerator Laboratory\\ 
Batavia, Illinois 60510, USA}
%
\affiliation[h]{
Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC- Universitat Polit\`ecnica de Val\`encia\\
Camino de Vera s/n, 46022 Valencia, Spain}
%
\affiliation[i]{
LIBPhys, Physics Department, University of Coimbra\\
Rua Larga, 3004-516 Coimbra, Portugal}
%
\affiliation[j]{
Donostia International Physics Center (DIPC)\\
Paseo Manuel Lardizabal 4, 20018 Donostia-San Sebastian, Spain.}
%
\affiliation[k]{
Lawrence Berkeley National Laboratory (LBNL)\\
1 Cyclotron Road, Berkeley, California 94720, USA}
%
\affiliation[l]{
Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela\\
Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, 15782 Santiago de Compostela, Spain}
%
\affiliation[m]
{Centro de Investigaci\'on en Ciencias B\'asicas y Aplicadas, Universidad Antonio Nari\~no\\ 
Sede Circunvalar, Carretera 3 Este No.\ 47 A-15, Bogot\'a, Colombia}
%
\affiliation[n]
{Argonne National Laboratory,\\ 
Argonne IL 60439, USA}
%
\affiliation[o]{
Department of Physics and Astronomy, Iowa State University\\
12 Physics Hall, Ames, Iowa 50011-3160, USA}
%
\affiliation[p]{
Department of Physics, University of Texas at Arlington\\
Arlington, Texas 76019, USA}
%
\affiliation[q]{
Departamento de F\'isica Te\'orica, Universidad Aut\'onoma de Madrid\\
Campus de Cantoblanco, 28049 Madrid, Spain}
%
\affiliation[r]{
Escola Polit\`ecnica Superior, Universitat de Girona\\
Av.~Montilivi, s/n, 17071 Girona, Spain}
%
\affiliation[s]{
Department of Physics and Astronomy, Texas A\&M University\\
College Station, Texas 77843-4242, USA}
%
%\affiliation[t]{
%Joint Institute for Nuclear Research (JINR)\\
%Joliot-Curie 6, 141980 Dubna, Russia}
%
\affiliation[t]{
IKERBASQUE, Basque Foundation for Science, 48013 Bilbao, Spain.}


==> pool/acknowledgments/ack.tex <==
The NEXT Collaboration acknowledges support from the following agencies and institutions: the European Research Council (ERC) under the Advanced Grant 339787-NEXT; the Ministerio de Econom\'ia y Competitividad of Spain under grants FIS2014-53371-C04 and the Severo Ochoa Program SEV-2014-0398; the GVA of Spain under grant PROMETEO/2016/120; the Portuguese FCT and FEDER through the program COMPETE, project PTDC/FIS/103860/2008; the U.S.\ Department of Energy under contracts number DE-AC02-07CH11359 (Fermi National Accelerator Laboratory), DE-FG02-13ER42020 (Texas A\&M) and de-sc0017721 (University of Texas at Arlington); and the University of Texas at Arlington. We acknowledge partial support from the European Union?s Horizon 2020 research and innovation programme through the RISE project InvisiblesPlus under grant agreement No 690575. Finally, special thanks are owned to the Laboratorio subterr\'aneo de Canfranc. 



==> pool/acknowledgments/ack2018.tex <==
The NEXT Collaboration acknowledges support from the following agencies and institutions: the European Research Council (ERC) under the Advanced Grant 339787-NEXT; the Ministerio de Econom\'ia y Competitividad of Spain under grants FIS2014-53371-C04 and the Severo Ochoa Program SEV-2014-0398; the GVA of Spain under grant PROMETEO/2016/120; the Portuguese FCT and FEDER through the program COMPETE, projects PTDC/FIS-NUC/2525/2014 and UID/FIS/04559/2013; the U.S.\ Department of Energy under contracts number DE-AC02-07CH11359 (Fermi National Accelerator Laboratory), DE-FG02-13ER42020 (Texas A\&M) and de-sc0017721 (University of Texas at Arlington); and the University of Texas at Arlington. We acknowledge partial support from the European Union?s Horizon 2020 research and innovation programme through the RISE project InvisiblesPlus under grant agreement No 690575. Finally, special thanks are owned to the Laboratorio subterr\'aneo de Canfranc. 



==> pool/acknowledgments/ack2018XeHe.tex <==
\section*{Acknowledgement}
The authors want to thank Igor Tolstikhin for providing useful references regarding helium diffusion through minerals. The NEXT Collaboration ac- knowledges support from the following agencies and institutions: the European Research Council (ERC) under the Advanced Grant 339787-NEXT; the Ministe- riodeEconom ́ıayCompetitividadofSpainundergrantsFIS2014-53371-C04, the Severo Ochoa Program SEV-2014-0398 and the Mar ́ıa de Maetzu Program MDM-2016-0692; the GVA of Spain under grants PROMETEO/2016/120 and SEJI/2017/011; the Portuguese FCT and FEDER through the program COM- PETE, projects PTDC/FIS-NUC/2525/2014 and UID/FIS/04559/2013; the U.S. Department of Energy under contracts number DE-AC02-07CH11359 (Fermi National Accelerator Laboratory), DE-FG02-13ER42020 (Texas A\&M) and de- sc0017721 (University of Texas at Arlington); and the University of Texas at Arlington. We acknowledge partial support from the European Union Horizon 2020 research and innovation programme under the Marie Sklodowska-Curie grant agreements No. 690575 and 674896. We also warmly acknowledge the Laboratorio Nazionale di Gran Sasso (LNGS) and the Dark Side collaboration for their help with TPB coating of various parts of the NEXT-White TPC. Finally, we are grateful to the Laboratorio Subterra ́neo de Canfranc for hosting and supporting the NEXT experiment.


==> pool/src/Krypton_selection_runII.tex <==
%\subsection{Selection of krypton candidates} 

\subsection*{Trigger}

\begin{figure}[tbh!]
  \begin{center}
    \includegraphics[width=0.4\textwidth]{pool/imgKr/s2u.png} \hfill
    \caption{\label{fig:s2u} Uncorrected S2 energy (in photoelectrons) measured by the sum of the PMTs. }
  \end{center}
\end{figure}

The detector triggers in the krypton \st\ signals. The uncorrected  energy of the \st\ signals depends quite strongly on \XYZ\, given the sizable effect of both the spatial (\XY) corrections and the lifetime. However, as illustrated in Figure \ref{fig:s2u}, the range of the total energy measured by the photomultipliers is well defined between \KrPmtSumEminRunII\ and \KrPmtSumEmaxRunII\ photoelectrons. The signal recorded in the 2 PMTs located at small radius is roughly 
\num{1/12} of the total energy. Thus, events are triggered if the signal in {\em both} central PMTs is in the range between \KrTriggerEminRunII\ and \KrTriggerEmaxRunII.

\subsection*{Waveform processing}

The raw data are PMT and SiPM waveforms. The PMT waveforms are sampled each \NewPMTSampling, while the SiPM waveforms are sampled each \NewSiPMSampling. The analysis proceeds according to the following steps.

\subsubsection*{Deconvolution of the PMT raw waveforms}

\begin{figure}[tbh!]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{pool/imgKr/rwf.png} 
    \includegraphics[width=0.45\textwidth]{pool/imgKr/cwf.png} 
    \caption{\label{fig:cwf} \Kr{83m} waveforms. Top panel: the raw waveform, showing the negative swing introduced by the PMTs front-end electronics. Bottom panel: corrected waveform.}
  \end{center}
\end{figure}

As described in [NEW], the PMT waveforms show a negative swing due to the effect of the front-end electronics. The first step in the processing is to apply a deconvolution algorithm [NEW, EPLANE], to the negative-swing, arbitrary-baseline, uncalibrated raw-waveforms (RWFs), to   produce positive-only, zero-baseline, calibrated waveforms (CWFs). Figure \ref{fig:cwf} shows the RWF and CWF waveforms corresponding to the sum of the PMTs in the energy plane. The event was triggered by the \st\ signal, which appears centered in the middle of the data acquisition window (DAQW). The \so\ signal appears at the beginning of the DAQW. 

\subsubsection*{Search for \so\ signals}

\begin{figure}[tbh!]
  \begin{center}
    \includegraphics[width=0.4\textwidth]{pool/imgKr/ns1.png} \hfill
    \caption{\label{fig:ns1} Number of \so\ candidates found by the peak-finding algorithm. }
  \end{center}
\end{figure}

\begin{figure}[tbh!]
  \begin{center}
    \includegraphics[width=0.9\textwidth]{pool/imgKr/s1histos.png} \hfill
      \caption{\label{fig:s1histos} Distributions of \so\ candidates, from left to right and from top to bottom: \SE, \SW, \SH\ and \ST. Blue (dashed) lines correspond to inclusive distributions (any number of \so\ candidates), black (solid) lines correspond to events with exactly one \so. Red (dot-dashed) lines correspond to events with 2 \so\ candidates and Green (dotted) lines to more than 2 \so\ candidates.}
  \end{center}
\end{figure}

The first half of the CWF (\eg\ drift time less than \KrSearchWindow) is processed by a peak-finding algorithm tuned to find small signals.  Each signal is characterized by its total energy (\SE), width (\SW), height (\SH) and time (\ST), defined as the time corresponding to its height. The output of the algorithm is a list of \so\ candidates. The distribution of the number of candidates is shown in figure \ref{fig:ns1}. A single \so\ is identified in about half of the events,  while 2 \so\ candidates are identified in near 30\% of the events and 3 or more candidates are identified in the remaining 20\% of the events. 
Figure \ref{fig:s1histos} shows the corresponding distributions. The 1-\so\ sample is dominated by genuine \so\ signals, the 2-\so\ sample usually includes a large signal associated to Krypton events happening in the field-cage buffer, and the multiple-\so\ sample is dominated by small scintillation signals which appear associated to \st\ signals (known as ``grass'' [REF]).  Consequently, the algorithm selects events with exactly one \so\ candidate.

The second half of the CWF (\eg\ drift time more than \KrSearchWindow) is then processed by the same peak finding algorithm, this time tuned to find larger signals. Most of the times a single \st\ candidate is found. Only events with exactly one \so\ and one \st\ are accepted for the analysis. Furthermore, a positive signal in at least one sensor of the tracking plane for the same time window of the \st\ is required. A SiPM is considered to have signal if the total charge in that time window exceeds \KrSiPMEminRunII. This threshold was taken to reduce the impact of SiPM dark noise at the operational temperature of the detector. 

\subsubsection*{Position of the event}

\begin{figure}[tbh!]
  \begin{center}
    \includegraphics[width=0.6\textwidth]{pool/imgKr/XY.png} \hfill
    \caption{\label{fig:xy} Distribution of events in the \XY\ plane. }
  \end{center}
\end{figure}

The \Z\ coordinate of the events is computed multiplying the drift time (obtained as the difference
between \ST\ for \so\ and \st) by the drift velocity. To obtain the transverse coordinates \XY\ of the event, a position-reconstruction algorithm integrated the charge recorded by the SiPMs of the tracking plane in the time window corresponding to the event \st. The position and charge of each SiPM (with charge above a threshold of \KrSiPmThreshold\, chosen to eliminate unwanted hits due to the SiPMs dark noise) enter into a barycenter algorithm that outputs the event position. Figure \ref{fig:xy} shows the distribution of events in the \XY\ plane. 
%The excess of events (yellow square) is due to a noisy SiPM.



==> pool/src/calibration_cs_th_sources.tex <==
\section{Calibrations with \CS\ and \TH\ radioactive sources}
\label{sec.calibCsTh}

\begin{figure}[!htb]
	\centering
	\includegraphics[width= 0.7\textwidth]{pool/imgThCs/TPC_config.pdf}
	\caption{Schematic of the source configuration in this study (not drawn to scale).  The \CS\ source was placed at the lateral entrance port of the pressure vessel, and the \TH\ source was placed on top of the pressure vessel.}\label{fig.config}
\end{figure}

Figure \ref{fig.config} shows the configuration of the \CS\ and \TH\ calibration sources used during Run II.  \CS\ decays by emitting a gamma ray with energy of approximately 662 keV, and \TH\ decays eventually to \TL\ which emits a gamma ray with energy of approximately 2615 keV. The \CS\,source was placed at the lateral port of the pressure vessel, and the \TH\, source was placed on top.  The trigger threshold was set low enough to capture events produced by both gamma rays simultaneously in the same acquisition.


\begin{figure}[!htb]
	\centering
	\includegraphics[width= 1.0\textwidth]{pool/imgThCs/CSTH_WF_run4735_evt149.pdf}
	\caption{The waveform of a calibration event with an approximate total energy of 1.6 MeV.}\label{fig.waveform}
\end{figure}

Interactions occurred in the drift region, producing ionization and primary scintillation.  Primary scintillation (\so) is detected first, and the time elapsed before detection of the EL scintillation (\st) was used to determine the z-coordinate at which the ionization was produced in the active region.
Figure \ref{fig.waveform} shows a typical waveform from a \TH\ event. The z coordinate is found from the distance between \so\ and \st. Then, the \st\ signal is sliced in \SI{1}{\mu s} slices. For each slice, a reconstruction algorithm records the SiPMs with charge in the tracking plane and determines the corresponding x-y coordinate. Thus, a 3D hit is built, where the tracking plane provides the transverse coordinates and the energy plane provides the longitudinal coordinates and the energy of the hit. Tracks are formed as collection of hits, and the energy of the track is obtained adding up the energy of all hits in the track.  



==> pool/src/effect_of_diffusion.tex <==
\section{The effect of diffusion in the track reconstruction}
\label{sec.diff}

In NEW (and NEXT-100), the \XY\ information comes directly from the light produced by the ionization electrons as they cross the EL gap, after drifting through the TPC active volume. As electrons travel through gas they diffuse in all dimensions, smearing the electron cloud produced by the interacting particle. As a result, the charge distribution arriving at the EL will be spread instead of concentrated at the interacting position of the particle, affecting the tracking power of the detector.

The impact of diffusion is qualitatively illustrated in Fig.~\ref{fig:track}. A simulated neutrinoless double beta decay (\bbonu) track from \XE\ (\XenonQbb\ deposited energy) interacting in xenon gas at \NewPressure\ is shown on the left panel of the figure. On the right panel, the same track is imaged after a \SI{40}{cm} drift distance, assuming the known diffusion parameters at that pressure, i.e. \simto \XenonLongitudinalDiffusion\ and \simto \XenonTransverseDiffusion\ for the longitudinal and transverse diffusion, respectively.

\begin{figure}[!htb]
  \begin{center}
%    \includegraphics[width=0.4\textwidth]{img/True_Track.pdf}
%    \includegraphics[width=0.4\textwidth]{img/Diff_Track.pdf}
 \caption{\label{fig:track} Simulated \XE\ \bbonu\ track assuming that no diffusion effects take place during the drift (left), and after drifting 40 cm assuming the longitudinal and diffusion coefficients to be 
 \XenonLongitudinalDiffusion\ and \XenonTransverseDiffusion\ respectively (right).}
  \end{center}
\end{figure}

Although the main feature needed to identify the track as two 
electrons (\eg\ the two high-energy deposition at the track end points) can still be seen, the picture is blurred due to the spreading of the ionization electrons, resulting in loss of information of the particle path. 




==> pool/src/hpxe_principle_of_operation.tex <==
\section{Principle of operation of \HPXeEL\ TPCs}
\label{sec.hpxe}

\begin{figure}[bhtp!]
\centering
\includegraphics[width=0.8\textwidth]{pool/imgNEXT/PrincipleOfOperation2.png}
\caption{\small Principle of operation of an \HPXeEL.} 
\label{fig.po}
\end{figure}

\Fig\ \ref{fig.po} illustrates the principle of operation of a high pressure xenon gas \HPXe. Charged tracks propagating in the TPC
lose energy  by ionizing and exciting the gas atoms. The latter will self-trap to form excimer states that de-excite by emitting vacuum ultraviolet (VUV) photons of \XeWaveLength\ wavelength. This prompt scintillation is the so-called primary signal (\so). 
The electrons produced by ionization along the track path will be drifted, under the influence of an electric field, towards the TPC anode.
In addition, the electric field reduces the effect of recombination to negligible levels for low ionization density particles like electrons at moderate pressures (<40 bar). The effects of recombination in xenon gas are only relevant for alpha particles where the ionization density is very high \cite{Alvarez:2012hu}.
 Near the anode, this delayed signal can be amplified by a variety of mechanisms. In the case of a \HPXeEL, the amplification is performed using electroluminescence (EL)~\cite{Aprile:2008bga}. A more intense electric field (of the order of \TypicalReducedField) is created in a region between the TPC gate, which is held at high voltage, and the grounded anode. This field strength accelerates the ionization electrons sufficiently to produce \st\ scintillation light. The EL field is kept low enough, below \MaximumLinealReducedField, to avoid additional gas ionization which would result in non-linearities in the amplification process. In the linear region, the reduced electroluminescent yield
(the number of photons produced per ionization electron entering the ELR, unit length and unit pressure),
$Y/P$, of an \HPXeEL\ can be empirically parametrized (\cite{Oliveira:2011xk}) as:
%
\begin{equation}
Y/P = (136 \pm 1) (E/P) - (99 \pm 4) {\rm ~[photons~electron^{-1}~cm^{-1}~bar^{-1}]}
\end{equation}
%
%
where $E/P$ is the reduced field in the ELR.

An  \HPXeEL\ is, therefore, an {\em optical TPC}, where both scintillation and ionization produce a light signal. In the NEXT detectors, the light is detected by two independent sensor planes located behind the anode and the cathode. The energy of the event is measured by integrating the amplified EL signal (\st) with a plane of photomultipliers (PMTs). This {\em energy plane} also records the \so\ signal which provides the start-of-event (\tz).  

EL light is also detected a few mm away from production at the anode plane by a dense array of silicon photomultipliers (SiPMs), known as the  \emph{tracking plane}. This measurement allows for topological reconstruction since it provides position information transverse to the drift direction. The longitudinal (or \Z) position of the event is obtained using the drift time which is defined as the time difference between the \so\ and \st\ signals. %In other words, the drift time is the time elapsed between the ionization time of the gas (marked by \so) and the time when the electrons reach the EL region (marked by \st).
%As \st\ light is produced in the EL region, near the sensors, \XY\ information transverse to the drift direction can be extracted from the SiPM response. The longitudinal (or \Z) position of the event can instead be obtained through the drift time, which is defined as the time difference between the \so\ and \st\ signals. In other words, the drift time is the time elapsed between the ionization time of the gas (marked by \so) and the time when the electrons reach the EL region (marked by \st). 


==> pool/src/intro_bbonu.tex <==
Neutrinoless double beta decay (\bbonu) is a hypothetical, very slow radioactive process in which two neutrons undergo $\beta$-decay simultaneously and without the emission of neutrinos. An unambiguous observation would establish that neutrinos are Majorana particles, identical to their antiparticles and would have deep implications in physics and cosmology. 
 
During the last decade several experimental programs deploying different technologies  and with masses in the ranges of few tens to few hundreds of kilograms have searched or are about to start searching for \bbonu\ processes~\cite{Gomez-Cadenas:2011it, Cremonesi:2013fa, DellOro:2016gf}.  Four of these experiments (GERDA~\cite{Agostini:2017fw}, EXO~\cite{Albert:2017tn}, KamLAND-Zen~\cite{Gando:2016br, Gando:2016ji}, and CUORE~\cite{Alduino:2017wj}) have recently published the results of their analysis, extending the sensitivity of previous searches by more than one order of magnitude.  Two more, NEXT~\cite{Gomez-Cadenas:2013lta} and SNO+~\cite{Andringa:2016gh}, will produce results in the next few years.
\par

==> pool/src/krypton_calibration.tex <==
\subsection* {Krypton calibrations in the \NEW\ detector}
\label{sec.krcal}

\begin{figure}[tbh!]
  \begin{center}
    \includegraphics[width=0.6\textwidth]{pool/imgKr/Rb_decay_scheme.png} \hfill
    \caption{\label{fig:Rb_decay_scheme} \Rb{83} decay scheme.}
  \end{center}
\end{figure}

Figure \ref{fig:Rb_decay_scheme} shows the decay scheme of a \Rb{83} nucleus. The exotic rubidium isotope decays to \Kr{83m} via electron capture with a lifetime of \RbLifetime. Krypton then decays to the ground state via two consecutive electron conversions releasing \KrEnergyI\ and \KrEnergyII, respectively. The decay rate is dominated by the first conversion with a half-life of \KrLifetime\ (the second one has a very short half-life of \KrLifetimeShort). The total released energy is \KrEnergy\ and the ground state of \Kr{83} is stable.

The rubidium source is a sample of small (a few mm diameter) porous zeolite balls, stored in a dedicated section of the gas system. \Kr{83m} nuclei produced after the electron conversion of \Rb{83} emanate from the zeolite and flow with the gas inside the chamber, spreading uniformly through the detection volume and producing point-like deposits of monochromatic energy (given the short half life of the second electron conversion, the measured energy of \Kr{83m} decays is \KrEnergy). The  source has an intensity of \RbIntensity. The rate of \Kr{83m} decays is limited by the data acquisition to a comfortable value of about  \KrRate. In addition, given the short half-life of \Kr{83m} the krypton activity is reduced to negligible levels a few hours after removing the rubidium source. 
\par


==> pool/src/krypton_data_periods.tex <==
\subsection*{Krypton data periods for \RII}
\label{sec.krp}

Krypton data for \RII\ were taken in two different periods. The first period ranged between \KryptonSevenBarStartRunII\ and \KryptonSevenBarEndRunII, at an operational pressure of \NewSevenBarPressureRunII. The second one occurred between \KryptonNineBarStartRunII\ and \KryptonNineBarEndRunII, at \NewNineBarPressureRunII. 
\par



==> pool/src/new_initial_operation_runII.tex <==
\section{Initial operation of the NEW detector: Run II}
\label{sec.operationRunII}

\begin{figure}[!htb]
\centering
\includegraphics[angle=0, width=0.99\textwidth]{runII/lifetime_kr}
\caption{Evolution of the lifetime during a fraction of Run II.} 
\label{fig.lifetime}
\end{figure}

After a short engineering run (Run I) in November-December 2016, the detector has been operating continuously since March 2017 (Run II). 

In order to assess the overall performance of the detector and the gas system while keeping a safety margin (\eg\ minimizing the effect of possible leaks as well as limiting the energy of potential sparks in the gate), the operational pressure in Run II was limited to \NewSevenBarPressureRunII\. The drift voltage was set at \NewDriftField\  and the reduced field in the EL region at \NewReducedFieldRunII, slightly below the nominal value of \NewReducedField. Thus, the gate voltage was kept at \NewGateVoltageRunII\ and the cathode voltage at
\NewSevenBarPressureRunII. Under those conditions, the chamber was extremely stable, with essentially no sparks recorded over the whole run. 

Towards the end of the run, the pressure was increased to \NewNineBarPressureRunII\ and the voltage in the gate (cathode) was increased to \NewGateVoltageRunIIMax\
(\NewCathodeVoltageRunIIMax). With the increased voltage a rate of a few sparks per week were  recorded. The sparks occurred in the mesh and the most likely reason appears to be burning of dust (an obvious possibility is TPB which ends up in the mesh when the chamber is heated to facilitate degassing). Inspection of the mesh and anode plate after Run II showed no damage in the mesh but small spots where the TPB and part of the ITO had been evaporated by the sparks were visible in the anode plate. On the other hand, the energy of the sparks can be quenched by coating the anode plate with a resistive material (such as PEDOT) rather than a conductor like ITO.   A new anode plate is consequently being fabricated with such an alternative coating and will be installed in NEW in the next few months. 

Electron lifetime appeared to be good (of the order of several milliseconds) during Run I, although the measurement was uncertain due to the evolving conditions of the chamber during that short period. Unfortunately, it was severely degraded at the beginning of Run II, possibly due to small oxygen leaks. This led to adding an exhaustive helium leak check of the full system before filling the chamber with xenon, which has been implemented for Run III now being prepared. On the other hand, the lifetime of the system could be improved by continuous gas circulation through the getters to an acceptable value of 2 ms. Figure \ref{fig.lifetime} shows the evolution of the lifetime during a fraction of the run. It is expected that the combination of a stringent detector tightness (guaranteed through the now-standard Helium test) and getter circulation will allow lifetimes comparable or larger than those achieved in Run I. 

Run II was mostly devoted to calibrations with radioactive sources, including \KR\, \NA, \CS\ and \TL\ sources. The primary goal was the overall characterization of the chamber, and an initial assessment of the energy resolution and topological signature. A first estimation of the background level in the detector was also made. 
%In the next section, we present a summary of the most important results obtained in Run II. A detailed discussion of those results will be subject of forthcoming publications. 

%Operation conditions: Pressure, HV, data taking


==> pool/src/new_overview.tex <==
\section {The NEW detector: an overview}
\label{sec.new}

\begin{figure}[bhtp!]
\centering
\includegraphics[width=0.99\textwidth]{pool/imgNEW/NEW.png}
\includegraphics[width=0.99\textwidth]{pool/imgNEW/NEW_cut_render.png}
\caption{\small Top: a diagram showing the main subsystems of the \NEW\ apparatus; bottom: a cut-away of the NEW detector.} \label{fig:NEW}
\end{figure} 

\begin{figure}[bhtp!]
\centering
\includegraphics[width=0.99\textwidth]{pool/imgNEW/NEW-castle.jpg}
\caption[caption for lof]{\small \NEW\ inside the lead shielding at the LSC. Picture from "\copyright www.jlarrea.com"} \label{fig:NEW2}
\end{figure} 



\begin{table}[htp]
%\caption{\NEW\ TPC parameters.}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
TPC parameter & Nominal & \RII (4734) & \RII (4841) \\
\hline
Diameter &  \multicolumn{3}{c|}{\NewTpcDiameter}  \\
Length & \multicolumn{3}{c|}{\NewTpcLength}  \\
Drift length & \multicolumn{3}{c|}{\NewTpcDriftLengthNoError}  \\
EL gap & \multicolumn{3}{c|}{\NewTpcELGap} \\\hline
Pressure & \NewPressure & \NewSevenBarPressureRunII & \NewNineBarPressureRunII \\
EL field (E/P) & \NewReducedField & \NewReducedFieldRunII & \NewReducedFieldRunII \\
%EL gap & \NewTpcELGap & \NewTpcELGap & \NewTpcELGap \\
$V_{gate}$ & \NewGateVoltageAtFifteenBar & \NewGateVoltageSevenBarRunII & \NewGateVoltageNineBarRunII\\
%Length & \NewTpcLength & \NewTpcLength & \NewTpcLength \\
%Diameter &  \NewTpcDiameter & \NewTpcDiameter & \NewTpcDiameter \\
Fiducial mass & \NewFiducialMass & \NewFiducialMassSevenBar & \NewFiducialMassNineBar\\
%Drift length & \NewTpcDriftLength & \NewTpcDriftLength & \NewTpcDriftLength \\
Drift field & \NewDriftField & \NewDriftField& \NewDriftField \\
$V_{cathode}$ &\NewCathodeVoltageAtFifteenBar &  \NewCathodeVoltageSevenBarRunII & \NewCathodeVoltageNineBarRunII\\
\hline%\hline
\end{tabular}
\end{center}
\caption{\NEW\ TPC parameters.}
%\caption{NEW TPC design parameters}
\label{tab.TPC}
\end{table}%


The \NEW\ apparatus, shown in figures \ref{fig:NEW}, \ref{fig:NEW2} is currently the world's largest radiopure \HPXeEL. Table \ref{tab.TPC} shows the main parameters of the TPC. The left column lists the nominal (design) parameters, while the center and right columns list the operational parameters during the initial operation of the detector (the so-called \RII\ described later in this paper). The
energy plane is instrumented with \NewNumberOfPMT\ \NewTypePMT\  PMTs located \NewCathodeToPMTs\ behind the cathode, providing a coverage of \NewPMTCoverage. The tracking plane is instrumented with \NewNumberOfSiPM\ SiPMs SensL series-C distributed at a pitch of \NewSipmPitch. An ultra-pure copper shell (ICS) \NewBarrelICS\ thick, acts as a shield in the barrel region. The tracking plane and the energy plane are supported also by pure copper plates \NewPlatesICS\ thick.  

% \begin{figure}[bhtp!]
%\centering
%%\includegraphics[width=0.9\textwidth]{pool/imgNEW/LSC-setup.png}
%\includegraphics[width=0.99\textwidth]{pool/imgNEW/NEW_cut_render.png}
%\caption{\small 
%%Top panel: a diagram showing the NEW detector and associated infrastructures at the LSC (the yellow beams mark the coverage of webcams for remote parameter control); bottom panel: 
%Transversal cut of the NEW detector.} \label{fig.newatlsc}
%\end{figure} 
 
%The detector operates inside a pressure vessel fabricated with a radiopure titanium alloy, \NewPressureVesselMaterial. The pressure vessel sits on a seismic table and is surrounded by a lead shield (the lead castle). Since a long electron lifetime is a must, the xenon circulates in a gas system where it is continuously purified. The whole setup sits on top of a tramex platform elevated over the ground at Hall-A, in the Laboratorio Subterr\'aneo de Canfranc (LSC) (figure \ref{fig.newatlsc}). 

The detector operates inside a pressure vessel fabricated with a radiopure stainless steel alloy (\NewPressureVesselMaterial). The pressure vessel sits on a seismic table and is surrounded by a lead shield (the lead castle). Since a long electron lifetime is a must, the xenon circulates in a gas system where it is continuously purified. The whole setup sits on top of a tramex platform elevated over the ground in HALL-A, at the LSC. 


==> pool/src/next_100.tex <==
\begin{figure}[hb!]
\centering
\includegraphics[width=0.9\textwidth]{pool/imgNext/next-100.png}
\caption{\small The \NEXT\ detector.}
\label{fig.next-100}
\end{figure}

The \Next\ detector, scheduled to be constructed in 2019, is an asymmetric high-pressure xenon electroluminescent (\HPXeEL) TPC shown schematically in figure \ref{fig.next-100}.  The fiducial region is a cylinder of \NextTpcDiameter\ diameter and \NextTpcLength\ length, (\NextFiducialVolume\ fiducial volume) holding a mass of \NextFiducialMass\ of xenon gas enriched at \XeEnrichment\ in \XE, and operating at \NextPressure.  The energy plane (EP), featuring \NextNumberOfPMT\ PMTs, provides a measurement of the energy integrating the full signal (\st).  It also records the primary scintillation light (\so) which triggers the start-of-event (\tz).  The tracking plane (TP) features an array of \NextNumberOfSiPM\ SiPMs. The SiPMs are \NextSiPMSizeTP\ sensors, manufactured by SENSL, with a PDE at \NextSiPMPeakPDEWavelength\ of \NextSipmPDE\ and a DCR of \NextSipmDCR\ at room temperature.  Screening of SiPMs only returned upper limits for contaminations in the main radioactive isotopes, indicating that SiPMs are very radiopure as expected of ultra-pure silicon dies.  The tracking plane provides a 2D image of the tracks propagating in the detector, which is then turned into a 3D image when combined with the measurement of the drift time.  

\begin{figure}[hb!]
\centering
\includegraphics[width=0.8\textwidth]{pool/imgNext/topo.png}
\caption{\small The \NEXT\ topological signature: the reconstruction of the trajectories of the electrons propagating in the gas permits to separate the two electrons emitted by a \bbonu\ decay (left panel) from single-electrons induced by backgrounds (right panel).}
\label{fig.topo}
\end{figure}

\begin{figure}[hb!]
\centering
\includegraphics[width=0.8\textwidth]{pool/imgNext/topoSel.png}
\caption{\small Separation between single electrons (left panel) and double electrons (right panel) in NEXT. A cut demanding large energy deposition in both track extremes (blob1 and blob2) allows an order of magnitude rejection of the background.}
\label{fig.topo2}
\end{figure}

The \HPXeEL\ technology combines {\em excellent energy resolution}, with an intrinsic limit of about \XenonIntrinsicEnergyResolution\ FWHM at \Qbb\ and an actual value of \NextBestEnergyResolution\ FWHM (for point-like energy depositions) as demonstrated with the operation of small prototypes~\cite{Alvarez:2013kh} and more recently with the  \New\ detector ~\cite{Martinez-Lema:2018ibw}. For long tracks, prototypes have shown a resolution of  
\NextLongTrackResolution, confirmed by recent \New\ results\footnote{J.J. Gomez-Cadenas, presentation to the scientific committee of LSC, April 2018, paper in preparation.}. Furthermore, the technology features 
a powerful {\em topological signature} (\fig\ \ref{fig.topo} and \fig\ \ref{fig.topo2}), capable of discriminating between signal (the two electrons emitted in a \bbonu\ decay) and background (mostly, single electrons induced by high energy gammas)~\cite{Ferrario:2016gf}.

The combination of excellent energy resolution and background rejection provided by the topological signature results in a very low background rate of \SI{5E-4}{counts\per\kg\per\keV\per\year}.  The projected background in the ROI for \Next\ is \SI{7}{\ev\per\tonne\per\yr}, with the leading background sources being the PMTs and the substrates of the SiPMs~\cite{GomezCadenas:2017vp}.  
%The sensitivity of \Next\ is expected to reach \SI{6E25}{\yr} with an exposure of \SI{300}{\kg\yr}. 

==> pool/src/ntk.tex <==
The \HPXeEL\ technology can be scaled up to multi-tonne target masses by introducing several new technological advancements \cite{Cadenas:2017vcu}.  These are:

\begin{itemize}

\item {\bf Construction of a Cold Gas Xenon (CGXe) TPC}, operating at \NtkOperatingTemperature, not far from the gas triple point.  Operation in this regime has two marked advantages: a) it reduces the DCR of the SiPMs by a factor \num{300} and b) it permits to operate at a lower pressure (\NtkOperatingPressure) than \Next\ (\NextPressure\ at \NextTemperature).  Reducing the pressure, in turn, simplifies the construction of future larger detectors required to perform a complete exploration of the IH discovery region.

\item {\bf Operation of the detector with a 0.85/0.15 xenon/helium mixture}.  As shown in Ref.~\cite{Felkai:2017oeq}, the addition of \SI{15}{\percent} of helium reduces the large transverse diffusion of natural xenon gas from \TransverseDiffusionPureXenon\ to \TransverseDiffusionXeHe, resulting in sharper reconstructed images for the electron trajectories and improving the performance of the topological signature by a factor \num{4}~\cite{Renner:2017ey}.

\item {\bf Replacement of PMTs with SiPMs}.  PMTs are the leading source of background in \Next\ and introduce scalability problems (operation in vacuum, risk of helium diffusion in the PMTs vacuum region, etc.).  Instead, SiPMs are intrinsically radiopure, resistant to pressure and able to provide better coverage.

\end{itemize}

The extrapolation of the technology to the tonne scale could proceed in two stages.  The first stage could upgrade the \NEXT\ detector to turn it into \NHD. This ``high definition detector'' would use a low diffusion gas mixtures and a dense tracking plane to improve the topological signature, and, depending of funding, could also increase the mass of \Next\ by a factor 3. The second stage would be \Ntk\, a symmetric CGXe TPC operating at \NtkOperatingTemperature\ with a mass of up to \NtkTotalMass\ (\NtkFiducialMass\ fiducial) when the gas is held at a pressure of \NtkMaximumPressure, corresponding to a density of \NtkMaximumDensity\ (see Figure~\ref{fig.n2k}). 
%\Ntk\ exploits the fact that the NEXT-100 pressure vessel and gas system is designed to withstand operation at \NextPressure, which is reached at \NtkMinimumTemperature\ when operating at \NtkMaximumPressure\ (thus allowing a comfortable margin of operation of \SI{10}{\K}).

\begin{figure}[t!]
   \begin{minipage}{0.58\textwidth}
     \centering
    \includegraphics[width=\linewidth]{pool/imgNext/n2.png}
     \caption{\small The \Ntk\ detector: a symmetric CGXe TPC. }
     \label{fig.n2k}
   \end{minipage}\hfill
   \begin{minipage}{0.40\textwidth}
     \centering
     \includegraphics[width=\linewidth]{pool/imgNext/n2-sector.png}
     \caption{\small \Ntk\ will have two identical sensor planes, alternating eSiPMs and tSiPMs mounted on ultra-pure substrates.}
     \label{fig.n2k-sipms}
   \end{minipage}
\end{figure}

\Ntk\ will feature two identical readout planes, located behind the two anodes (Figure~\ref{fig.n2k-sipms}).  The planes alternate large-area SiPMs (\SI[product-units=power]{10 x 10}{\square\mm}), called energy-SiPMs (eSiPMs), with small-area SiPMs (\SI[product-units=power]{1 x 1}{\square\mm}), called tracking-SiPMs\ (tSiPMs).  Both eSiPMs and tSiPMs are placed at a pitch of \SI{11}{\mm}. 

\Ntk\ will reduce the background rate of \Next\ by more than one order of magnitude, due to the combination of the improved topological signature, providing a factor of~\num{4} extra rejection against backgrounds, and of a background budget at least a factor of~\num{3} smaller than that of \Next, achieved thanks to the elimination of the two leading sources of radioactivity, \eg, PMTs and the tracking plane Kapton boards in use for the mounting of SiPMs.  At the same time, \Ntk\ can deploy a mass twice as large as that of \Next.  The target background of \Ntk\ is \SI{<1}{\ev\per\tonne\per\yr}, allowing the experiment to reach a sensitivity of \SI{1E27}{\yr} in \Tonu\ with an exposure of \SI{5.0}{\tonne\yr}.  This performance would improve the current state of the art by a factor of~\num{10}, opening the possibility for a discovery.  

%Importantly, all the crucial technology improvements for \Ntk\ {\em can be demonstrated} by suitable upgrades of the \Next\ detector, which would permit to test each of the crucial steps leading to the ton-scale technology, namely cool gas operation, SiPM as energy sensors, low diffusion mixtures and barium tagging. 



%In addition, \Ntk\ will be the first step to construct larger detector(s) with masses in the tonne range, ultimately able to push the sensitivity to \mbb\ by an additional order of magnitude, thus allowing the complete exploration of the IH discovery region.


==> pool/src/the_search_for_bbonu.tex <==
The only practical way to determine if neutrinos are Majorana particles, identical to their own antiparticles, is to observe neutrinoless double beta decays (\bbonu), a nuclear transition, $(Z,A) \rightarrow (Z+2,A) + 2\ e^{-}$, in which a nucleus with $Z$ protons decays into a nucleus with $Z+2$ protons and the same mass number $A$, {\em without emitting neutrinos}. The simplest mechanism to mediate such a transition is the virtual exchange of light Majorana neutrinos. Assuming this exchange to be  dominant at low energies, the half-life of \bbonu\ can be written as:

\begin{equation}
(T^{0\nu}_{1/2})^{-1} = G^{0\nu} \ \big|M^{0\nu}\big|^{2} \ \mbb^{2}; \,\,\, \,\,
\mbb = \Big| \sum_{i} U^{2}_{ei} \ m_{i} \Big|
\label{eq:mbb}
\end{equation}

where $G^{0\nu}$~ is a phase-space integral for the emission of two electrons, $M^{0\nu}$ is the nuclear matrix element (NME) of the transition, and \mbb\ is the \emph{effective Majorana mass} of the electron neutrino, defined in terms of the neutrino mass eigenstates ($m_{i}$) and the elements of the neutrino mixing matrix ($U_{ei}$)~ \cite{GomezCadenas:2012fe}.

\begin{figure}[hb!]
\centering
\includegraphics[width=0.5\textwidth]{pool/imgNext/landscape.png}
\caption{\small The effective neutrino mass \mbb\ as a function of the mass of the lightest neutrino.  The current generation of experiment will explore the so-called ``degenerate neutrino mass region'', up to $\mbb \simeq \SI{50}{\meV\per\square\c}$.  The target of the next generation is to explore the inverse hierarchy, in the range from \SIrange{20}{50}{\meV\per\square\c}.}
\label{fig:Majorana-Landscape}
\end{figure}

When \mbb\ is represented as a function of the lightest neutrino mass, ${\rm m_{light}}$~as in the left panel of Figure~\ref{fig:Majorana-Landscape}, one obtains the ``Majorana landscape'' defining the space of opportunity for discovery.  This landscape is being explored by the current generation of \bbonu\ experiments, achieving exposures in the range of hundred  kilogram~year\cite{Cadenas:2017vcu,Cremonesi:2013fa,DellOro:2016gf}\ Four of these experiments (GERDA~\cite{Agostini:2017fw, Agostini:2018tnm}, EXO~\cite{Albert:2017tn}, KamLAND-Zen~\cite{Gando:2016br,Gando:2016ji}, and CUORE~\cite{Alduino:2017wj}) have recently published the results of their analysis, extending the sensitivity of previous searches by more than one order of magnitude.  Two more, NEXT~\cite{Cadenas:2017vcu} and SNO+~\cite{Andringa:2016gh}, will produce results soon.  The best limit on the lifetime of a \bbonu\ isotope was obtained by KamLAND-Zen~\cite{Gando:2016br,Gando:2016ji}), corresponding to $\Tonu > \KZenTz$ for the \bbonu\ decay of \XE.  This translates into a sensitivity to the effective neutrino mass of \KZenMbb, almost scratching the upper limit of the so-called inverse hierarchy (IH) of neutrino masses ordering. The other experiments now leading the field (GERDA, EXO, CUORE, NEXT and SNO+) expect to reach a similar sensitivity level in the next few years. 

Notice that the redundancy provided by different experiments with similar ultimate sensitivity is a strong asset for the field due to the fact that it permits: a) to explore several isotopes (specifically \GE, \TL\ and \XE) and b) to produce a robust result when several experiments per isotope are available as in the case of Xenon, given the very different background models and systematic errors of the involved experiments. Indeed, KamLAND-Zen  strategy is based in large-mass and powerful self-shielding, in exchange or poor energy resolution, while NEXT approach maximizes energy resolution (plus the availability of a topological signature) in exchange of a more modest mass (EXO is in between the KamLAND-Zen and the NEXT techniques, featuring some self-shielding and modest resolution). In particular, both KamLAND-Zen and EXO must handle a substantial background count in their regions of interest (ROI) near \Qbb\ (of the order of 10 events while NEXT-100 aims to less than one background count per year in the ROI. As further discussed below, discovery in \bbonu\ searches all but requires background-free experiments. The capability of NEXT-100 to provide such a near background free experiment at the 100 kg scale and the potential (also further discussed below) to improve its radioactive budget, resolution and topological signature so that background free experiments at the ton scale are also possible, is the strongest asses of the experiment and have placed NEXT among the three experiments (together with GERDA and CUORE) identified by APPEC as having the strongest potential for the future of \bbonu\ searches in Europe\footnote{http://www.appec.org/wp-content/uploads/Documents/Current-docs/APPEC-Strategy-Book-Proof-19-Feb-2018.pdf}

The next step for the field is to fully explore the IH discovery region.  This requires to push the sensitivity to \IHMass.  Given the quadratic dependence of \mbb\ upon the inverse of the lifetime,  increasing the sensitivity to \mbb\ by a factor of~\num{3} requires building experiments with a sensitivity to \Tonu\ of \IHTz. Exploration of the normal hierarchy (NH) requires an ultimate sensitivity to \mbb\ of \NHMass, which translates into a sensitivity to \Tonu\ of \NHTz.

The obvious implication is that the next generation of experiments sailing to explore the IH will require a growth in exposure of at least one order of magnitude.  Yet this alone is not sufficient, since the sensitivity to \Tonu\ grows linearly with exposure, implying that the sensitivity for \mbb\ grows with the square root of exposure $\sqrt{Mt}$, {\bf only for background-free experiments}; instead, in presence of background, the sensitivity improves only with $\sqrt[4]{Mt}$.

\begin{figure}[hb!]
\centering
\includegraphics[width=0.5\textwidth]{pool/imgNext/sensi-xenon.png}
\caption{\small Sensitivity of a fully efficient \XE\ experiment as a function of the exposure, for different background rates.}
\label{fig.Xe}
\end{figure}

The detrimental effects of the presence of background are illustrated by Figure~\ref{fig.Xe}, which shows the sensitivity to \mbb\ (using a reasonable set of nuclear matrix elements) of a fully efficient \XE\ experiment as a function of exposure, for different background rates.  A fiducial exposure of almost \SI{2}{\tonne\yr} (corresponding to an actual exposure of \SI{5}{\tonne\yr}, when accounting for efficiency of the detector) is required for a full exploration of the IH region {\em in the background free case}, \eg, for \BackgroundFreeLimit\ of background.  The exposure increases to \SI{3}{\tonne\yr} (\SI{8}{\tonne\yr}) for \AlmostBackgroundFreeLimit\ of background and degrades rapidly for larger backgrounds.  Thus, the conclusion is that the next generation of \bbonu\ experiments must feature target masses in the tonne-range, while keeping the total background contained within \AlmostBackgroundFreeRequirement. 



==> src/Commands.tex <==
\newcommand{\Ba}[1]{\ensuremath{^{#1}\mathrm{Ba}}\xspace}
\newcommand{\Bi}[1]{\ensuremath{^{#1}\mathrm{Bi}}\xspace}
\newcommand{\Co}[1]{\ensuremath{^{#1}\mathrm{Co}}\xspace}
\newcommand{\Cs}[1]{\ensuremath{^{#1}\mathrm{Cs}}\xspace}
\newcommand{\Kr}[1]{\ensuremath{^{#1}\mathrm{Kr}}\xspace}
\newcommand{\Na}[1]{\ensuremath{^{#1}\mathrm{Na}}\xspace}
\newcommand{\Pb}[1]{\ensuremath{^{#1}\mathrm{Pb}}\xspace}
\newcommand{\Po}[1]{\ensuremath{^{#1}\mathrm{Po}}\xspace}
\newcommand{\Rb}[1]{\ensuremath{^{#1}\mathrm{Rb}}\xspace}
\newcommand{\Rn}[1]{\ensuremath{^{#1}\mathrm{Rn}}\xspace}
\newcommand{\Th}[1]{\ensuremath{^{#1}\mathrm{Th}}\xspace}
\newcommand{\Tl}[1]{\ensuremath{^{#1}\mathrm{Tl}}\xspace}
\newcommand{\U}[1]{\ensuremath{^{#1}\mathrm{U}}\xspace}
\newcommand{\Xe}[1]{\ensuremath{^{#1}\mathrm{Xe}}\xspace}
%\newcommand{\Kr}[1]{\ensuremath{^{#1}\mathrm{Kr}}\xspace}
%\newcommand{\Kr}[1]{\ensuremath{^{#1}\mathrm{Kr}}\xspace}



\newcommand{\bbnonu}{\ensuremath{\beta\beta0\nu}\xspace}
\newcommand{\bbtwonu}{\ensuremath{\beta\beta2\nu}\xspace}
\newcommand{\bb}{\ensuremath{\beta\beta}\xspace}
\newcommand{\Qbb}{\ensuremath{Q_{\beta\beta}}\xspace}






==> src/checks.tex <==
\section{\label{sec:checks} Checks and Systematic uncertainties}

\subsection{lifetime}

TODO: distribution of the standardized residuals (is a pull?), 
TODO: compare maps obtained for different z range [50, 200], [200, 350] [350, 500]
TODO: how the lifetime maps evolve? Inside a run, between different runs!

\subsection{geometrical}

TODO: distribution of the geometrical corrections from two different runs, how does it compare
TODO: distribution of the geometrical corrections from different z-regions

\subsection{energy resolution}

TODO: vary the selection: S1 width, S1 charge, S2 charge, how does this affect the e-res in z, r?
TODO: vary the lifetime-map, how does this affect the e-res?
TODO: vary the geo-map, how this affect the e-res?


==> src/data.tex <==
\section{\label{sec:data} Data}

The data used in this analysis has been collected with NEXT-White during the summer and autumn 2017. The list of runs is listed in Table \ref{tab:data}. The trigger rate was 7.9 Hz. In approximately 24 hours, we collected a million of triggers. 

%%%
\begin{table}[tbh]
\caption{\label{tab:data} Run conditions}
\begin{center}
\begin{tabular}{cccccc}
\hline
Run    & Date               & Triggers & Pressure & $\Delta V_{\mathrm{drif}t}$ & $\Delta V_{\mathrm{EL}}$ \\
           &                       & (M)              & (bar)        & (kV)                     & (kV) \\ \hline
4628   &  7/9   - 11/9   &  2.443    &  7.18            & 28                       & 7 \\ 
5734   &  7/10 - 10/10 &  2.687     & 7.16              & 28                       & 7 \\
\end{tabular}
\end{center}
\end{table}
